An EM Framework for Online Incremental Learning of Semantic Segmentation

Incremental learning of semantic segmentation has emerged as a promising strategy for visual scene interpretation in the open- world setting. However, it remains challenging to acquire novel classes in an online fashion for the segmentation task, mainly due to its continuously-evolving semantic label space, partial pixelwise ground-truth annotations, and constrained data availability. To ad- dress this, we propose an incremental learning strategy that can fast adapt deep segmentation models without catastrophic forgetting, using a streaming input data with pixel annotations on the novel classes only. To this end, we develop a uni ed learning strategy based on the Expectation-Maximization (EM) framework, which integrates an iterative relabeling strategy that lls in the missing labels and a rehearsal-based incremental learning step that balances the stability-plasticity of the model. Moreover, our EM algorithm adopts an adaptive sampling method to select informative train- ing data and a class-balancing training strategy in the incremental model updates, both improving the e cacy of model learning. We validate our approach on the PASCAL VOC 2012 and ADE20K datasets, and the results demonstrate its superior performance over the existing incremental methods.

==> data/__latexindent_temp.tex <==
\textit{4) Herding} strategy aims to find an image subset whose feature mean over pixels in the feature space is the most close to the mean of the entire dataset of that class.
Table.~\ref{tab:memory_strategy} summarizes the result about memory selection strategies.
Surprisingly, random sampling, despite its simplicity,  is consistently better than other memory selection strategies including the complex herding strategy on all budgets.

==> data/methods.tex.tex <==
\section{Our approach}\label{sec:approach}


In this section, we introduce our learning strategy for incremental semantic segmentation, which aims to continuously learn novel visual concepts for pixel-wise semantic labeling of images. 
In particular, given a sequence of semantic classes, we consider the task of building a segmentation model in multiple incremental \remove{steps}\myadd{tasks}, and in each \remove{step}\myadd{task}, the model needs to be updated for an
expanded semantic label space with only limited data memory of previous \remove{steps}\myadd{tasks}. 
In this limited-memory setting, our goal is to achieve efficient adaptation of the segmentation model without catastrophic forgetting of previously learned semantic classes. 


To this end, we develop an incremental learning approach for deep segmentation networks based on the Expectation-Maximization (EM) framework. Our EM learning method incorporates a re-labeling strategy for augmenting annotations and an efficient rehearsal-based model adaptation with dynamic data sampling within a single framework.  
Such an integrated framework enables us to cope with the challenges of catastrophic forgetting, efficient model adaptation, and background concept drift simultaneously and in a principled manner.
% The organization
Below we start with an introduction of our problem setting in Sec. \ref{subsec:setup}, followed by a formal description of our model architecture in Sec. \ref{subsec:model_arch}.
Then we present our EM-based incremental learning approach in Sec. \ref{subsec:em_framework}.
% and a warm start technique for the EM learning in Sec. \ref{subsec:warm_start}
\subsection{Problem Setup}\label{subsec:setup}
%In this work, we aim to address the incremental semantic segmentation problem. In particular, we learn the system which could fast updates itself with a stream of data.
%Concept:
%Step, classes, images, labels(partial)
%Goal: optimization with constraint
%Step0 
%Our model $\mathcal{M}_t$ observes a stream of data over steps $t$ where the training data $D^{tr}_t=\{X_t,Y_t,C_t\}$ $X_t$ means the training images, $Y_t$ represents the corresponding annotations where only $\{x_i:c(x_i) \inC_t\}$ are labeled and $C_t$ is the novel categories to recognize.
% The model observes a stream of data
The task of online incremental semantic segmentation typically starts from a base task $\mathcal{T}_0=\{\mathcal{D}^{tr}_0,\mathcal{Y}_0\}$ in which $\mathcal{D}^{tr}_0$ is the training dataset, and $\mathcal{Y}_0$ are the base semantic classes. We denote the {background class} of $\mathcal{T}_0$ as $U_0$, which includes all the irrelevant classes not in $\mathcal{Y}_0$, and $\tilde{\mathcal{Y}}_0=\mathcal{Y}_0\cup \{U_0\}$ are the categories including background class at the initial \remove{step}\myadd{task}. 
The initial training set $\mathcal{D}^{tr}_0=\{(\mathbf{x}^0_i,\mathbf{y}^0_i)\}_{i=1}^{|\mathcal{D}^{tr}_0|}$, where $\mathbf{x}_i^0\in\mathbb{R}^{H\times W \times 3}$ and $\mathbf{y}_i^0\in \tilde{\mathcal{Y}}_0^{H\times W}$ are the $i$-th image and its fully-labeled annotation, respectively. For the base task, we assume a segmentation model $\mathcal{S}_0$ has been trained on $\mathcal{D}^{tr}_0$. 

%system
During the incremental learning stage, the \remove{system}\myadd{pretrained segmentation model} receives a stream of new semantic class groups $\{\mathcal{C}_t\}_{t\geq 1}$ and their corresponding training data $\{\mathcal{D}^{tr}_t\}_{t\geq 1}$.
For task $t$, the data comes as a stream of mini-batch $B^{tr}_i=(\bm{X}_i, \bm{Y}_i)$  in an online manner where $\bm{X}_i$ means a set of images and $\bm{Y}_i$ is its corresponding annotation.
%Compared to offline learning, online learning is bounded by run-time and capability of lifelong learning with limited data, which is more realistic and human-like.
In other words, the model is only allowed to use the incoming batch $B^{tr}_i$ to update its parameters only once(up to k times).
\myadd{
We assume a small set of exemplars from previous steps (up to $t$) can be stored in an external memory, denoted as $\mathcal{M}_t$, and can be used for training the segmentation model $\mathcal{S}_t$. 
Typically, samples are drawn from memory and concatenated with the incoming batch.}
%How to convey: the union of batches is the complete training set.
At each incremental task $t$, we assume that only pixels from the novel classes  are labeled, which may be caused by lacking previous labeling expertise and/or limited annotation budget. 
%$\mathcal{D}^{tr}_t$ \mathcal{D}
Specifically, the incoming training data $B^{tr}_k$ has a form of $\{(\mathbf{x}^t_i,\mathbf{y}^t_i, \mathcal{R}^t_i)\}_{i=1}^{|B^{tr}_k|}$ at task $t$, in which $\mathbf{y}^t_i$ is the partial annotation, and $\mathcal{R}^t_i$ indicates the labeled region in the image $\mathbf{x}^t_i$. 
For each pixel $j\in \mathcal{R}^t_i$, we have its label $\mathbf{y}^t_{i,j}\in \mathcal{C}_t$ and otherwise $\mathbf{y}^t_{i,j}$ is unlabeled. 


Our goal is to learn an updated segmentation model $\mathcal{S}_t$ to incorporate the novel semantic classes in $\mathcal{C}_t$, and to achieve strong performance on a test data $\mathcal{D}^{ts}_t$. 
We note that $\mathcal{D}^{ts}_t$ includes all the semantic classes up to the $t$-th task, denoted as $\mathcal{Y}_t=\mathcal{Y}_0\cup\left(\cup_{\tau=1}^t\mathcal{C}_\tau\right)$, and the corresponding \textit{background class} $U_t$.% from $\{\mathcal{D}^{tr}_t\}_{t=0}^t$ and $\mathcal{M}_{t-1}$.      


%\myadd{with less training FLOPs consumption}.\myadd{Besides $\mathcal{D}^{tr}_t$, we also have exemplars from previous steps saved as memory $\mathcal{M}_t$ for training $\mathcal{S}_t$.}

% Original
%\modify{As the pixelwise annotation is costly to obtain in a typical semantic segmentation task, we adopt a novel incremental learning setting in this work. In particular, we assume all the annotated data up to the step $t$ can be stored in an external memory, denoted as $\mathcal{M}_t$, and can be used for training $\mathcal{S}_t$. However, in each step $t$, we have a computation budget $\mathcal{B}_t$, measured as total FLOPs, to update the model $\mathcal{S}_t$ from $\mathcal{S}_{t-1}$, which limits the amount of data used in the actual training.}

%In particular, the goal is to optimize the performance at any step for all observed lasses $\cup_{0\le i \le T} C_i$ where $T$ is the number of observed steps.

\begin{figure*}[t]
%	\hspace{-3mm}
	\begin{minipage}{0.47\linewidth}
		\centering
		%\resizebox{\textwidth}{!}{
		\begin{algorithm}[H]
			\caption{The Method Overview.}
			\hspace*{-0.2em} {\bf Initialize:} Model $\mathcal{S}_0$; Memory Size $|\mathcal{M}|$; Memory $\mathcal{M}_0=$$\text{Random Sample}(\mathcal{D}^{tr}_0;|\mathcal{M}|)$
			\begin{adjustwidth}{-1em}{}
				\begin{algorithmic}
					\For{\texttt{$t=1,2,3...$}}
					\State \textcolor{gray}{// warm start}
					\State Select $D_c$ from $\tilde{\mathcal{D}^{tr}_t} = \{\mathcal{M}_{t-1}, \mathcal{D}^{tr}_t \}$	
					\State Extract Conv features $\mathcal{V}_c\!=\!\{\mathcal{F}_{t-1}(\bm{x}_i)\!:\!\bm{x}_i\in D_c \}$ 
					\State Finetune segmentation head $\mathcal{H}_t$ with $\mathcal{V}_c$
					\State \textcolor{gray}{// incremental learning with EM}
					\While{The budget $\mathcal{B}_t$ is not used up}
					\State Run EM iteration in \textbf{Algorithm} \ref{alg:em}.
					\EndWhile
					\State $\mathcal{M}_t$$=$$\text{Random Sample}(\mathcal{M}_{t-1},\mathcal{D}^{tr}_t;|\mathcal{M}|)$
					\EndFor
				\end{algorithmic}
			\end{adjustwidth}
			\label{alg:overview}
		\end{algorithm}
	\end{minipage}
	\hspace{5mm}
	\begin{minipage}{0.47\linewidth}
		\centering
		%\resizebox{\textwidth}{!}{
		\begin{algorithm}[H]
			\caption{The EM Iteration.}
			\hspace*{0in} {\bf Input:} The model $\mathcal{S}$; Step $t$; Batch-size $B$
			\begin{adjustwidth}{-0.9em}{}
				\begin{algorithmic}
					\State \textcolor{gray}{// sample images to build mini-batch $\mathcal{N}_t$}
					\State $\mathcal{N}_t = \emptyset$
					\For{\texttt{$k=1,2,3...,B$}}
					\State Sample the class $c_{k}$ according to $P_s(c)$ (Eq. \ref{eq:3})
					\thickmuskip=0.5\thickmuskip
%					\State $D_s\!=\!\{(x_l,y_l,R_l)\in \mathcal{M}_{t}|\{j|\bm{y}_{l,j}\!=c_{k},j\!\in\!\mathcal{R}_l\}\neq\!\emptyset\}$
					\State Denote $D_s\!=\!\{(\bm{x}_l,\bm{y}_l,\mathcal{R}_l)\in \mathcal{M}_{t}|\,\exists j\in \mathcal{R}_l,\,\bm{y}_{l,j}=c_k\}$
					\State Uniformly sample $(\bm{x}_i,\bm{y}_i,\mathcal{R}_i)$ from $D_s$
					\State $\mathcal{N}_t = \mathcal{N}_t \cup \{i\}$
					\State Refine label $\bm{y}_i$ by relabeling (Eq. \ref{eq:4})

					\EndFor
					\State Update model $\mathcal{S}$ with the loss $\mathcal{L}$ (Eq. \ref{eq:5})
					\State Update class sampling probability $P_s(c)$ (Eq. \ref{eq:3})
				\end{algorithmic}
			\end{adjustwidth}
			\label{alg:em}
		\end{algorithm}
	\end{minipage}
\end{figure*}

\subsection{Model Architecture}\label{subsec:model_arch}
%\paragraph{Model Architecture}
<<<<<<< HEAD
For each task $t$, we assume a typical semantic segmentation network architecture, which consists of an encoder-decoder backbone network $\mathcal{F}_t$ extracting a dense feature map and a convolution head $\mathcal{H}_t$ that produces the segmentation score map. Note that our method is agnostic to specific network designs.
=======
For each \remove{step}\myadd{task} $t$, we assume a typical semantic segmentation network architecture, which consists of an encoder-decoder backbone network $\mathcal{F}_t$ extracting a dense feature map and a convolution head $\mathcal{H}_t$ that produces the segmentation score map. Note that our method is agnostic to specific network designs.
>>>>>>> bed53a885c955f5dcdaeca5fdd4a6bf0a87a2bbd

Concretely, given the image $\mathbf{x}_i$, the segmentation network first computes the convolutional feature map $\mathbf{F}_i\in\mathbb{R}^{H\times W\times D}$ using the backbone network, where $D$ is the number of channels. $\mathbf{F}_i$ is then fed into the $1\times 1$ convolution head $\mathcal{H}_t$, which has a form of linear classifier at each pixel location. Denote the parameters of the backbone network as $\mathbf{W}_t^b$, and the parameters of head as $\mathbf{W}^h_t\in \mathbb{R}^{D\times(|\mathcal{Y}_t|+1)}$, our network generates its output $\mathbf{\hat{y}}_i$ as follows, 
\begin{align}
&\mathbf{F}_i=\mathcal{F}_t(\mathbf{x}_i;\mathbf{W}^b_t), \\
&p(\mathbf{\hat{y}}_i|\mathbf{x}_i)=\text{\small{Softmax}}(\mathcal{H}_t(\mathbf{F}_i))=\prod_{j\in\Omega_i}p(\mathbf{\hat{y}}_{ij}|\mathbf{F}_{ij};\mathbf{W}^h_t) 
\end{align}
where $\Omega_i$ represents the 2D image plane and $\mathbf{F}_{ij}\in \mathbb{R}^{D}$ for the pixel $j$. 
%Here for each pixel at $j$, we have a probability vector $p(\mathbf{\hat{y}}_{ij}|\mathbf{F}_{ij};\mathbf{W}^h_t) = \text{\small{Softmax}}(\mathbf{W}_t^{h\intercal}\mathbf{F}_{ij})$  with dimension $|\mathcal{Y}_t|+1$, where $\mathbf{\hat{y}}_{ij}\in \tilde{\mathcal{Y}}_t=\mathcal{Y}_t\cup \{U_t\}$ which includes the background at step $t$. 

%\paragraph{Memory Design} Considering the memory cost is cheap in many scenarios like data center, and the annotation is pretty valuable, we relax the memory constraint compared with previous works\cite{ozdemir2018learn,ozdemir2019extending,cermelli2020modeling,michieli2019incremental,tasar2019incremental}. Specifically, we store all observed data as memory for rehearsal.

\subsection{Incremental Learning with EM}\label{subsec:em_framework}

We now develop an EM learning framework to efficiently train the model $\mathcal{S}_t$ at the \remove{step}\myadd{task} $t$ with a limited memory $\mathcal{M}_t$ and a computation budget $\mathcal{B}_t$. To tackle the stability-plasticity dilemma, our strategy integrates the ideas in rehearsal-based learning and pixel relabeling, which enables us to efficiently re-use the training data for fast model adaptation and cope with background drift caused by the partial annotation. 

Specifically, we formulate the problem as learning with latent variables and develop a stochastic EM algorithm to iteratively update the model parameters. 
In each iteration, our EM algorithm first samples a mini-batch of training images, then fills in the missing labels and finally trains the model with one step of SGD.
%The learning procedure iterates through those three stages. : 1) dynamic sampling mini-batch of training data; 2) an E-step that relabels pixels with missing or background annotations, and 3) an M-step that updates the model parameters with one step of SGD. 
 Below we assume an initial parameter $\bm{\theta}_t$ and describe the details of the three stages in each EM iteration. A complete overview of our algorithm is shown in Algorithm~\ref{alg:overview}.

%When only the annotation for the novel classes pixels is available
%Specifically, we can observe the image values $\bm{X}$ and the corresponding annotation $\bm{Y}$, but the background pixels at initial step $0$ and the unlabeled pixels at incremental steps $t>0$ are regarded as latent variables $\bar{\bm{Y}}$. 

\paragraph{Dynamic sampling}

The first stage is to sample a mini-batch $\mathcal{N}_t$ of training data for a single step in the subsequent EM update. Our goal is to achieve efficient model updates to learn the new classes but also to retain old ones. To this end, we develop a dynamic sampling strategy that only selects a small set of informative training data for an EM iteration. 

Specifically, we devise a category-level sampling strategy that attempts to balance the training samples from the novel classes to be learned and the old ones prone to model forgetting. Concretely, our method maintains a  \textit{class sampling probability} $P_s(c)$ for $\forall c\in \tilde{\mathcal{Y}}_t$, which will be described below. In order to sample a training image, we first sample a class label $c_i$ according to $P_s$, and then uniformly sample an image $\mathbf{x}_i$ that has pixels labeled with $c_i$. 
%Formally, denote the set of semantic classes in the annotation $\mathbf{y}_i$ as $\mathcal{V}_i\subset \mathcal{Y}_t$, and the sampling probability can be written as,
%\begin{align}
%p_s(\mathbf{x}_i) = \sum_{c\in\mathcal{Y}_t}\text{Uniform}(\mathbf{x}_i|c\in\mathcal{V}_i)p_s(c). 
%\end{align}
Such a sampling process allows the model to visit certain classes more frequently to improve their learning. 

Our key design is to dynamically update the class probability $P_s$ according to the prediction confidence in the outputs of current model $\mathcal{S}_t$. 
To achieve this, we first compute an estimate of class confidences, denoted as $\{E(c),c\in\tilde{\mathcal{Y}}_t\}$, at each iteration of EM. Concretely, we use a moving average to collect the statistics from mini-batches as follows,
\begin{align}
E(c) &= \mu E_{{old}}(c) + (1-\mu)E_{mb}(c), \quad  \\
E_{mb}(c) &= \underset{{i\in \mathcal{N}_t, \mathbf{{y}}_{i,j}=c}}{\text{Mean}}\{p(\mathbf{\hat{y}}_{i,j}=c|\mathbf{x}_i;\bm{\theta}_t^{old})\}
\end{align}
where $E_{old}$ and $E_{mb}$ denotes the confidence estimate from last iteration and current mini-batch, respectively, $\mu$ is the momentum coefficient, and $\bm{\theta}_t^{old}$ is the model parameters from last iteration. At the beginning of each incremental step $t$, we initialize $E(c)$ as $0$ for all the class in $\tilde{\mathcal{Y}}$.   

Given the class confidences, we define the sampling probability $P_s$ with a Gibbs distribution, which assigns higher sampling probability to the classes with lower confidence:  
\begin{align}
P_s(c) = \frac{e^{-\eta E(c)}}{\sum_{k=1}^{|\tilde{\mathcal{Y}}_t|} e^{-\eta E(k)}} \quad \forall c\in \tilde{\mathcal{Y}}\label{eq:3}
\end{align}
where $\eta$ is the hyperparameter to control the peakiness of the distribution.


\paragraph{E-step}

In E-step, we tackle the problem of background concept drift due to the expansion of semantic label space $\mathcal{Y}_t$, and exploit the unlabeled regions in the training data of incremental steps for model adaption. To this end, we treat the labels of the background pixels in $\{\mathcal{D}^{tr}_0\}$ and the unlabeled pixels in $\{\mathcal{D}^{tr}_t\}_{t\geq 1}$ as hidden variables, and use the current model to infer their posterior distribution given the images and semantic annotations. We then use the posterior to fill in the missing annotations for the subsequent model learning in the M-step. By augmenting the training data with those pseudo labels, we aim to further improve the training efficiency and alleviate the problem of inconsistent background annotation.     

Specifically, given a training pair $(\mathbf{x}^\tau_i, \mathbf{y}^\tau_i), i\in \mathcal{N}_t$, in our sampled mini-batch, we first compute an approximate posterior of the latent part of $\mathbf{y}^\tau_i$. Here $\tau\in\{0,\cdots,t\}$ indicates the incremental step it comes from. Denote the region with latent labels as $\bar{\mathcal{R}}^\tau_i$, the posterior of its $j$-th pixel can be estimated as   
$p(\mathbf{\hat{y}}_{i,j}|\mathbf{x}^\tau_i;\bm{\theta}_t^{old})$ based on the current network. We then generate a pseudo labeling for those pixels by choosing the most likely label predictions as follows,
\begin{align}
\mathbf{{y}}^\tau_{i,j} = \underset{\mathbf{\hat{y}}_{i,j}\in\mathcal{\tilde{Y}}_t - \mathcal{C}_\tau}{\arg\max} p(\mathbf{\hat{y}}_{i,j}|\mathbf{x}^\tau_i;\bm{\theta}_t^{old}), \quad j\in \bar{\mathcal{R}}^\tau_i
\label{eq:4}
\end{align}
where $\mathcal{C}_\tau$ is the class group from step $\tau$. To filter out unreliable estimation, we only keep the pseudo labels of those pixels with confidence higher than a threshold $\delta$, i.e., $p(\mathbf{{y}}^\tau_{i,j}|\mathbf{x}^\tau_i;\bm{\theta}_t^{old})>\delta$. We adopt this hard EM to update our model in the next stage.    


\paragraph{M-step}

Our M-step employs the mini-batch training data with augmented annotations to update the model parameters. In order to fully utilize the image annotations, we propose a composite loss consisting of two loss terms as follows, \begin{align}
\mathcal{L} = &- \sum_{i\in \mathcal{N}_t} \sum_{\mathbf{{y}}^\tau_{i,j}\in\mathcal{\tilde{Y}}_t} \log p(\mathbf{{y}}^\tau_{i,j}|\mathbf{x}_i^\tau;\bm{\theta}_t) \\
	&- \gamma\sum_{i\in \mathcal{N}_t} \sum_{j\in\bar{\mathcal{R}}^\tau_i} \log \sum_{\mathbf{{y}}^\tau_{i,j}\notin \mathcal{C}_\tau} p(\mathbf{{y}}^\tau_{i,j}|\mathbf{x}_i^\tau;\bm{\theta}_t)
\label{eq:5}
\end{align}
where $\gamma$ is a weighting coefficient. The first term is the standard cross-entropy loss on every pixel with real annotation or pseudo labels, while the second term penalizes the model on classifying the unlabeled pixels at step $\tau$ into label space $\mathcal{C}_\tau$, which encourages the labeling consistent with the partial groundtruth annotations.


\subsection{Class Balancing Strategies}
We introduce our strategies to deal with the class-imbalance issues in the online class-incremental semantic segmentation problem. We first present the cosine normalization and then introduce the class-balanced exemplar selection strategy in this subsection.

\paragraph{Cosine Normalization}For the prediction of each pixel at $j$, we have a probability vector $p(\mathbf{\hat{y}}_{ij}|\mathbf{F}_{ij};\mathbf{W}^h_t)$ with dimension $|\mathcal{Y}_t|+1$ where k-th element is as follows
\begin{align}
	p(\mathbf{\hat{y}}^k_{ij}|\mathbf{F}_{ij};\mathbf{W}^h_t) = \frac{e^{\tau d(\bm{u}_k , \mathbf{F}_{ij})}}{\sum_{c=1}^{|\mathcal{Y}_t|+1} e^{\tau d(\bm{u}_c , \mathbf{F}_{ij})}}
\end{align}
%\overline{\mu}_k, 
%\sum_{c=1}^{|\mathcal{Y}_t|+1} e^{\tau <\overline{\mu}_k, \mathbf{F}_{ij}>
%\mathbf{W}}^{hk}_t}
where $\tau$ is the temperature used to control the sharpness of the softmax distribution, $u_k\in\mathbb{R}^D$ is the k-th column of classifier weight $\mathbf{W}^h_t$, and $d$ means the cosine distance metric.
%\text{\small{Softmax}}(\mathbf{W}_t^{h\intercal}\mathbf{F}_{ij})
%, where $\mathbf{\hat{y}}_{ij}\in \tilde{\mathcal{Y}}_t=\mathcal{Y}_t\cup \{U_t\}$ which includes the background at step $t$. 
It is worth noting that we are the first to adopt cosine normalization in the online class incremental learning problem, even though there has been works adopting it in many other problems\cite{luo2018cosine,qi2018low}.



\paragraph{Class-balanced Exemplar Selection} 
% Motivation of class-balanced memory.

% 
We extend the CBRS(class-balanced reservoir sampling)~\cite{} into the incremental semantic segmentation problem by considering the multiple instances of different classes in the image.
Therefore, we update the memory to make it as class-balanced as possible.
We pre-allcoate a size for each class.We allocate nearly same memory size for each class.
The streaming data is highly temporally correlated.
We apply reservoir sampling for each class.

%encourages the model to predict labeling consistent with partial annotations on unlabeled pixels.}
%Binary Classification
%the second term is a regularization term to discourage model classifying the unlabeled pixels on images of step $\tau$ into label space $\mathcal{C}_\tau$.}
%\remove{
%\subsection{Warm Start}\label{subsec:warm_start}
%% Motivation of warm start(Why we optimize head at first for each step)
%As the EM learning can be sensitive to the model initialization, we propose a light-weight warm-start strategy to generate an initial model parameter $\bm{\theta}_t$. Specifically, we directly copy the backbone network from last step, $\mathbf{W}^b_t = \mathbf{W}^b_{t-1}$, and only finetune the head $\mathcal{H}_t$ with a small subset of training data randomly selected  from the entire dataset $\tilde{\mathcal{D}^{tr}_t}=\mathcal{D}^{tr}_t \cup \mathcal{M}_t$. During our finetuning, we also cache the feature maps ($\mathbf{F}_i$) of the selected subset to save the computation.}  

